VEglue: Testing Visual Entailment Systems via Object-Aligned Joint Erasing

Visual entailment (VE) is a multimodal reasoning task consisting of image-sentence pairs whereby a promise is defined by an image, and a hypothesis is described by a sentence. The goal is to predict whether the image semantically entails the sentence. VE systems have been widely adopted in many downstream tasks. Metamorphic testing is the commonest technique for AI algorithms, but it poses a significant challenge for VE testing. They either only consider perturbations on single modality which would result in ineffective tests due to the destruction of the relationship of image-text pair, or just conduct shallow perturbations on the inputs which can hardly detect the decision error made by VE systems. Motivated by the fact that objects in the image are the fundamental element for reasoning, we propose VEglue, an object-aligned joint erasing approach for VE systems testing. It first aligns the object regions in the premise and object descriptions in the hypothesis to identify linked and un-linked objects. Then, based on the alignment information, three Metamorphic Relations are designed to jointly erase the objects of the two modalities. We evaluate VEglue on four widely-used VE systems involving two public datasets. Results show that VEglue could detect 11,609 issues on average, which is 194%-2,846% more than the baselines. In addition, VEglue could reach 52.5% Issue Finding Rate (IFR) on average, and significantly outperform the baselines by 17.1%-38.2%. Furthermore, we leverage the tests generated by VEglue to retrain the VE systems, which largely improves model performance (50.8% increase in accuracy) on newly generated tests without sacrificing the accuracy on the original test set.

==> sec/backup.tex <==
0726

\section{Introduction}
\label{sec:introduction}

\jie{comment}
%我不是特别确定，我们这里要不要先说一两句更大一点的背景，例如大模型在各个方面整表现出卓越的能力，它的推理能力还相对比较欠缺，也是很多研究的关注重点。这其中，涉及到多模态的推理是一个更有挑战性的领域，因为他涉及到不同模态的信息理解和融合等等，VE干嘛干嘛。
%这样可能显得你这个事情更重要一些。
%写VE任务的重要性
Visual Entailment (VE) aims to reason about the relationship between an image and a text \cite{ning2018visual,ning2019visual}.
% Specifically,  given an image as a premise, and a natural language sentence as a hypothesis，
% the VE model understands the content of the premise and the hypothesis and determine if premise can be concluded by the hypothesis.
Specifically, given an image as the premise, and a sentence in natural language as the hypothesis, the Visual Entailment (VE) determines whether the hypothesis logically follows from the premise and outputs their relationship, i.e., entailment, neutral, or contradiction.
% the Visual Entailment (VE) model comprehends the contents of both the premise and the hypothesis.
% Subsequently, it 
% Specifically, given an image as a premise $P$, and a natural language sentence as a hypothesis $H$, the VE model determine if $H$ can be concluded by the $P$.
% There are three labels (entailment, neutral, contradiction) are assigned based on the relationship conveyed by the $(P, H)$.
% Entailment means the content of the $P$ logically implies the meaning of the $H$.
% Neutral indicates that there is no clear visual evidence in the $P$ to determine the truth of the $H$. 
% Contradiction signifies a direct conflict or inconsistency between the visual content of an $P$ and the meaning of a $H$.
% As the input to the VE task is multimodal data, it plays a crucial role in bridging the gap between computer vision and natural language understanding. 
\yang{As a fundamental task in the multimodal learning field, VE affects many downstream tasks such as Image Captioning~\cite{peter2018bottom,xiao2022scaling}, Visual Question Answering~\cite{stan2015vqa,Yash2019making,qing2021check}, and Image-Text Retrieval~\cite{manh2023hada}, and is applied in many real-world scenarios such as of fake news detection~\cite{Shreyash2022FACTIFY, Suryavardan2022Factify2}, medically assisted diagnosis \cite{YanakaNCK23}, and auto-driving \cite{liang2023visual}.}
% Moreover, it affects many downstream multimodal tasks such as Image Captioning \cite{peter2018bottom,xiao2022scaling}, Visual Question Answering \cite{stan2015vqa,Yash2019making,qing2021check}, and Image-Text Retrieval \cite{manh2023hada}. 
% When the image and text representations within a news item are inconsistent, it has the potential to mislead or harm viewers. 
% Such inconsistencies can be effectively identified using VE models, thereby mitigating the spread of misinformation.
Therefore, ensuring the quality of the VE model is of significant importance.

%写测试VE任务的重要性，写一些VE错误导致的安全性问题
% With the rapid growth of social media, fake news is proliferating and can be very harmful.
% For example, a news report shows an image of a person not smoking, but the text description says the person is smoking. Such inconsistencies between the text description and the image content are often misleading or malicious, and thus require critical Content moderation. 
% The VE task plays a crucial role in identifying and addressing these inconsistencies \cite{Shreyash2022FACTIFY, Suryavardan2022Factify2}. Therefore, ensuring the quality of the VE model is of significant importance.
\begin{figure}[t]
\centering
\includegraphics[width=8cm,height=3cm]{fig/motivation.png}
\caption{The original and transformed premise-hypothesis pairs and the corresponding relationships
}
\label{fig:motivation}
\end{figure}


\yang{
As the premise for the VE task, an image contains many regions of interest that refer to different elements in the real world, such as persons, dogs, birds, walls, etc.
Similarly, the hypothesis also expresses some objects and their associated properties, as well as some textual elements with less information to ensure the grammaticality and fluency of the whole sentence, such as conjunctions, prepositions, etc.
As reported by Xie et al, different types of elements take discrepant effects for the VE task, where the involving \textit{objects}\footnote{we follow the definition of ``objects'' for VE task in the previous study~\cite{LinMBHPRDZ14}.} serve as the foundation to reason about final relations~\cite{ning2019visual}.
Take the sample in Figure \ref{fig:motivation} as an example.
The premise contains the three conspicuous objects, i.e., ``a girl'', ``a boy'', and ``a door'', as well as their surrounding contexts, i.e., ``the wall'' and ``the floor''.
While the hypothesis likewise describes two objects and their features, i.e., ``a girl stands nearby'' and ``a boy sits''.
Following the general paradigm of relation inference in the VE task, on the premise side, the model will detect and encode the region of objects (the three objects framed in red) within the premise.
On the hypothesis side, the VE model will pointedly encode the key textual elements, typically referring to the objects and their associated feature descriptions, using the attention mechanism.
After that, the VE will conduct relation inference based on the semantic logic of the two-sided encoding.
Therefore, noise that occurs to the objects in either premise or the hypothesis may be more likely to result in performance fluctuation.
Accordingly, introducing object-centric perturbations is a promising strategy to expose issues for VE models.
}
% \jie{comment}
%noise that occurs to the objects' region in the premise 这个说法，会让我误以为，你要变的是object's region，感觉像是在这个object区域附近加些噪声还是怎么着的。这里是不是就直接说改变这个object，要不感觉有点误导。


% 


\yang{
In recent years, many perturbation techniques are proposed for  deep learning testing in the literature.
Considering the input modalities in the VE task, the general perturbation techniques for images and texts could potentially be applied in VE testing.%第一段补一下多模态测试方法没有
However, these techniques commonly fall short when dealing with the VE task due to two aspects.
First, the vast majority of existing studies conduct semantically-equivalent perturbation, to ensure that the semantics does not change substantially before and after the perturbations.
For example, image-oriented perturbations include blurring, fogging, rotation, scaling, etc.
As for texts, the widely-used perturbation techniques are based on synonym substitution, back translation, simulating some character-level spelling errors, or removing some uninformative words (e.g., adverbs and conjunctions).
These perturbations are relatively subtle and shallow, which can hardly affect the issue detection ability of the automated testing approaches.
Especially for the VE task, these techniques ignoring the effects of objects are not likely to challenge the model's inference capacities. %intro最前面加推理能力
Second, some techniques conduct some deeper perturbations, such as adding some objects to the images or inverting the semantics of text by adding some negative words.
Since these techniques are oriented to a single modality and do not consider the semantic correlation between multimodal data.
The arbitrary perturbations to the data on either side may break the consistency on the other side, resulting in incorrect test inputs.
In summary, object-centric perturbation techniques considering the semantic relevance between two modalities are a crucial factor in VE testing in terms of  both the correctness of test generation and the effectiveness of issue detection.
}


% To the best of our knowledge, there are no test approaches for VE models. 
% The input for VE models consists of data from two modalities.
% Perturbations to one modality (either image or text) can also be used in VE models. 
% \jie{comment}
%我觉得这个说法有点不太通顺，可能要加点过渡。can also be used这个逻辑有点奇怪。要不要就说，VE涉及到text和image，已有研究分别有针对image的技术和针对text的技术，然后介绍下相关技术。到最后再说目前没有同时考虑两个方面的perburbations。
% Existing testing approaches \cite{HendrycksD19} for computer vision (CV) tasks apply uniform transformations to all regions of the image, such as blurring or fogging.
% Such methods only apply perturbations to the image without considering text information, and the degree of perturbation in the object regions is low, resulting in insufficient issue detection capabilities.
% While existing testing approaches \cite{JiangBTZD21} for natural language processing (NLP) tasks transform words in the text while preserving the semantic meaning, also only considering information from the text without the image.
% Besides, the perturbed words are not necessarily concentrated on the keywords describing the objects, resulting in limited issue detection capabilities under the VE task.
% Therefore, performing perturbations in conjunction with the objects is an effective way to detect issues in VE models.
% Therefore, combining image and text information to perturb the objects could be more effective in detecting VE model issues.

% In Figure \ref{fig:motivation}, the two object descriptions in the hypothesis correspond with two object regions in the premise, thus the relationship between the premise and the hypothesis is determined as entailment.
% Inspired by the VE model design concept, We believe that introducing perturbations around the object information in images and text is an effective strategy to identify issues in VE models.
% As one of the basic input elements in the VE task, the premise, i.e. image, typically contains multiple semantic elements, mainly divided into objects and their surrounding context.
% Xie et al. \cite{ning2019visual} represent the objects in the VE model as the Region of Interest (ROI) detected by the CNN \cite{GirshickDDM14} network, which is the foundation of VE model reas oning.
% In addition, the hypothesis, expressed in natural language, is composed of descriptions of the objects and their associated features.
% Besides, the hypothesis, i.e. natural language, is composed of descriptions of the objects and their corresponding actions.
% The VE model determines whether the hypothesis can be concluded given the semantic elements of the premise.
% Given the left half of Figure \ref{fig:motivation} as an example.
% The premise contains the girl, the boy, and the door as objects as well as the wall and the floor as backgrounds.
% The hypothesis includes descriptions of two objects, i.e. ``girl stands nearby'' and ``boy sits''.
% These two parts of the description correspond to two of the three objects in the premise.
% Thus the model infers an entailment relationship between the premise and the hypothesis.
% The premise includes multiple contents, including objects that people often focus on (the girl, the boy, and the door), as well as the background outside of these objects (the wall and the floor).
% The hypothesis expressed in natural language typically describes the objects in the image (``girl stands nearby'' and ``boy sits'').
% The VE model  determine whether the hypothesis can be concluded given the contents in the premise, which is based on the understanding of the objects.
% Xie et al. \cite{ning2019visual} represent the objects in the VE model as the region of interest (ROI) detected by the CNN \cite{GirshickDDM14} network, i.e., categories of objects that people define as common in life, such as people, bicycles, birds, etc.
% In this paper, we follow the widely-used object categories defined in \cite{LinMBHPRDZ14}.
% The semantics in the hypothesis typically describes the objects on the image.
% The VE model for reasoning about the relationship between images and text requires first extracting features of the object region in the image and features of important keywords describing the object in the text, respectively \cite{ning2019visual}.



% The most relevant task to the VE task is the Textual Entailment (TE) task, from which the VE task is derived \cite{DaganGM05}.
% The premise and hypothesis of the TE task are in natural language, and there are proposed test methods under that task that can be migrated to the VE task.
% Wang et al. \cite{WangLGZZZYZZPWL21} proposed to change the premise-hypothesis relationship into a contradiction by changing numbers in the text or reversing the gender words in the text.
% However, this type of approach is designed to be rule-specific and can only generate a limited number of test cases under the VE task, thus detecting fewer issues.
% Jiang et al. \cite{JiangBTZD21} proposed to perform synonym substitution on hypothetical texts without changing the relationship between the generated premise-hypothesis pairs.
% This approach does not do synonym transformation around the words describing the object in the text and may do perturbation on some non-object describing words which have a low impact on the model inference, so the generated test cases are not efficient in discovering the issues.
% This approach only introduces the semantically-equivalent perturbation at the word level in the text, which implies a lesser degree of impact on the text compared to perturbing the entire object description within the text.
% Therefore, its issue detection capability is insufficient.
% As for images, the state-of-the-art testing method is to insert an object in the background of an image to generate a new test case \cite{YuZQYWH22}.
% However the generated test cases suffer from unnaturalness and are less likely to be encountered in reality,  As a result, they are not well-suited for VE tasks that require reasoning about realistic images and texts.
%这个理由不知道能否站住脚
% For the widely-used image perturbation method \cite{HendrycksD19}, its issue detection ability is limited because of its application of global uniform perturbations to the image, without specifically focusing on the objects within the image.

%而想对检测的目标设计蜕变规则，存在两个挑战，挑战一是将图片中的区域和文本中的语义子单元结合，挑战二是如何对这些对应的目标物体做蜕变，生成自然的测试套件。


Metamorphic testing has been widely applied to test deep learning models in the test oracle problem due to its simplicity of concept and effectiveness in issue detection~\cite{ChenKLPTTZ18}.
The core of metamorphic testing is a set of Metamorphic Relations (MRs), which are necessary properties of the tested model in relation to the inputs and their expected output.
\yang{
In the VE testing, when designing reasonable MRs, it is essential to understand the logical relationship between input perturbation and corresponding test oracle.
Generally, objects described in the hypothesis are usually a subset of objects in the premise.
Given correspondence between premises and hypotheses, some of the objects in the premise are represented in the hypothesis (denoted as \textit{linked objects}), while others are not (denoted as \textit{non-linked objects}).
On the one hand, perturbations to different types of objects have discriminative effects on the test oracle.
For the premise in Figure \ref{fig:motivation}, the girl and the boy belong to the linked objects while the door falls non-linked objects.
If we erase a linked object, i.e. the girl or the boy, in the premise and leave the hypothesis unchanged, the test oracle will change from entailment to contradiction.
Otherwise, if the erasing operation occurs in the non-linked object, i.e. the door, the test oracle will remain entailment.
The fact motivates us to build the object-level links between the premise and the hypothesis to distinguish the linked and non-linked objects in the premise.
On the other hand, the range of perturbations, i.e., perturbations on a single side or on both sides, also has a significant effect on the test oracle.
Specifically, if we erase the girl in the premise and simultaneously remove the relevant description in the hypothesis (transform the original hypothesis into ``a boy sits''), the test oracle still remains entailment.
Therefore, the design of the metamorphic rule should comprehensively consider the object type, perturbation range, and their influence on the test oracle.
}

To ensure the rationality of MRs, when applying metamorphic testing to multimodal tasks like VE, it's essential to understand how perturbations to the test input (either premise or hypothesis) affect the changes in the test oracles (i.e., relationships).
It is the first challenge when conducting object-centric perturbations in the VE task.
%以图一为例，将为什么要关联图像对象和文本语义单元，因此文本图像有联系，所以对图像改变会改变关系
There are two types of inputs in the VE model and they are related to each other. 
Therefore, perturbing the objects in only one of the inputs cannot guarantee the relationship between the two.
% Due to the connection between objects in images and text, perturbing objects in images can affect the relationship.
Taking Figure \ref{fig:motivation} as an example, the region of the girl in the image disappears after perturbation and the semantic unit in the hypothesis keeps unchanged.
The semantic unit represents a description of an object in a hypothesis.
Since this object was originally associated with the semantic unit (``girl stands nearby'') in the hypothesis, perturbing this object region changes the relationship to ``contradiction''.
If the girl's region is not associated with the semantic unit, it's hard to determine the changes in the relationship between the premise and the hypothesis.
% Without associating the girl region with the semantic unit, changes in the relationship between premises and assumptions cannot be identified.
Therefore, only after associating the objects in the image with the semantic units in the hypothesis can we capture the impact of objects' perturbations on the relationship.
% if the region where the girl in the premise image is located is not associated with a semantic unit (``girl stands nearby'') in the hypothesized text, then after making a perturbation of the girl in the image, it is not known whether the perturbation affects the original relationship, and thus it is not possible to provide the relationship between the newly generated premise-hypothesis pairs.
% The first challenge is connecting the object region in the premise with the corresponding semantic units in the hypothesis that describe a specific object within the image.
% Designing metamorphic testing under the VE task requires determining whether perturbations to objects affect the test oracle, i.e., the relationship between the premise and the hypothesis.
% Therefore, it's necessary to establish the correspondence between objects in the premise and hypothesis in order to determine whether perturbations to an object will affect their relationship.
% Without establishing this connection, it would be impossible to determine whether the relationship between the premise-hypothesis pair would be affected by the transformation made to the object.
% Taking Figure \ref{fig:motivation} as an example, if the region where the girl in the premise image is located is not associated with a semantic unit (``girl stands nearby'') in the hypothesized text, then after making a perturbation of the girl in the image, it is not known whether the perturbation affects the original relationship, and thus it is not possible to provide the relationship between the newly generated premise-hypothesis pairs.
In addition, to ensure the correctness of the MR design, it is necessary to generate correct test inputs.
Under the VE task, the objects in the image and the surrounding contexts are closely connected, and perturbing the object region needs to ensure the naturalness and integrity of the surrounding context.
Similarly, in hypothesis, perturbation of semantic units needs to maintain the fluency and semantic integrity of the original hypothesis.
Therefore, it is challenging to generate correct and natural test inputs when conducting object-centric perturbations.
% Since the objects in images and semantic units in the text contain surrounding contexts.
% To generate correct test inputs, it's crucial to maintain the integrity of these contexts in both the image and the text without causing any disruptions.
% For instance, in Figure \ref{fig:motivation}, the removal of an object in the image does not affect the overall naturalness and integrity of the image.


%我们提出了一种针对检测目标的图文结合的蜕变测试方法，首先将文本分为若干语义子单元，然后根据视觉定位模型将每个语义子单元和图像上的区域关联，之后设计多个蜕变测试规则，对图像上的目标做删减，最终生成测试套件
To address the above challenges, we propose a jointly object-centric perturbation approach (named {\tool}) for VE testing.
{\tool} first extracts semantic units from the input hypothesis through the Large Language Model.
Subsequently, {\tool} uses a Visual Grounding model to determine the correspondence between the semantic units and the object regions in the image.
Simultaneously, {\tool} identifies potential object regions in the image, and in conjunction with the object regions already matched to semantic units, it discerns object regions that are irrelevant to the semantic units.
After confirming the relationship between image objects and semantic units, {\tool} designs three MRs based on whether the association between the object and the semantic unit is changed or not, i.e., simultaneous perturbations applied to both objects and semantic units (MR1), perturbations on objects associated with semantic units (MR2), and perturbations on objects unrelated to semantic units (MR3).
% Among them, MR1 and MR3 do not change the original relationship, while MR2 changes the original relationship to ``contradiction''.
For perturbing the objects in the image, {\tool} employs image inpainting techniques \cite{SuvorovLMRASKGP22} to remove them, to ensure the naturalness of the premise after perturbation.
As for perturbing the semantic unit, {\tool} removes it from the original hypothesis and does semantically-equivalent perturbation of the remaining semantic units, to increase the degree of perturbation while increasing the fluency of the hypothesis. 

% Under the framework of metamorphic testing, {\tool} introduces three MRs, i.e., simultaneous perturbations applied to both objects and semantic units, perturbations on objects associated with semantic units, and perturbations on objects unrelated to semantic units.
% Specifically, through semantic unit extraction, image-aware region localization, and object detection, {\tool} could connect semantic units with object regions on an image.
% Then, for perturbing the objects in the image, {\tool} employs image inpainting techniques \cite{SuvorovLMRASKGP22} to remove them, to ensure the naturalness of the premise after perturbation.
% As for perturbing the semantic unit, after it is deleted, {\tool} conducts the semantically-equivalent perturbation to the remaining semantic units, to ensure the semantic integrity of the hypothesis after perturbation.

%我们的方法比基线高XXX，能检测出多少缺陷，并且方法在重新训练后能极度减少之前存在的缺陷
We evaluate the issue detection capability of {\tool} on two publicly available VE datasets, i.e, SNLI-VE \cite{ning2018visual} and e-SNLI-VE \cite{Virginie2020esnlive}. 
We test on the state-of-the-art VE model (OFA \cite{WangYMLBLMZZY22}). 
The experimental results show that the {\tool} reports 10852 issues, and the Error Finding Rate (EFR) is 6.6\%-40.1\% higher than by baselines.
In addition, when testing the SOTA VE models, the test cases generated by the MR in the {\tool} achieved an EFR of 76.2\%.
Furthermore, we leverage the test cases generated by {\tool} to retrain the VE model, which largely improves model robustness (0\%-0.4\% EFR) while maintaining the accuracy of the original test set.
The key contributions of this paper are as follows:
%我们方法的贡献：1）第一个针对视觉推理任务提出的蜕变测试方法，达到了XXX的性能 2）成功将检测目标和文本相结合，成为后续针对检测目标设计蜕变规则的前提； 3）设计多个针对目标的蜕变规则，生成自然的测试套件 4）开源代码和数据，为后续的工作提供insight。
\begin{itemize}
    \item
    We propose a jointly object-centric pertubation approach for Visual Entailment testing by connecting image objects and textual semantic units and designing Metamorphic Relations that do not change the context of premises and hypotheses.
    Moreover, this is the first approach for testing the VE model considering the two modes (image and text), to the best of our knowledge, and can motivate other research related to multimodal learning models. 

    \item 
    We perform comprehensive experiments to evaluate the effectiveness of {\tool}, the experimental results show that {\tool} can obviously improve the issue detection ability and significantly outperforms the state-of-the-art baselines on two widely used datasets.
    
    \item
    By fine-tuning the original model with the generated tests, the performance of the VE model could be significantly improved.
   
    \item
    We provide the public reproduction package\footnote{https://github.com/lsplx/VEtesting} including the tool implementation and datasets.
\end{itemize}



Backgournd-20230727
\section{Background and Motivation}
\label{sec:background}
\subsection{Visual Entailment}
%介绍这个任务，并讲清楚VE模型的原理
Visual Entailment (VE) is in the field of multimodal learning that aims to understand the relationship between a given premise (serving as an image) and a hypothesis (serving as a text) \cite{ning2018visual,ning2019visual}.
The task is framed as a ternary classification problem with the classes being entailment, contradiction, and neutral.
We will use the example in Figure \ref{fig:motivation} to elaborate on the three relationships in the following.

\begin{itemize}
    \item 
    \textbf{Entailment:} It means the content of the premise logically implies the meaning of the hypothesis. 
    The premise in the example contains a girl and a boy, which is semantically consistent with what is described in the hypothesis, and therefore the relationship should be entailment.
    \item 
    \textbf{Contradiction:} It signifies a direct conflict or inconsistency between \rev{the visual content of} a premise and \rev{the meaning of} a hypothesis.
    Premise-2 in the example contains only a boy, while the hypothesis describes two objects, i.e., ``a boy'' and ``a girl''.
    \rev{while a girl is mentioned in the hypothesis text, which makes an obvious contradiction between the premise and the hypothesis, and} 
    Therefore the relationship between the two is a contradiction.
    \item 
    \textbf{Neutral:} It indicates that there is no clear \rev{visual} evidence in the premise to determine the truth of the hypothesis. 
    Using Premise-1 as an example, the corresponding hypothesis is changed to ``a girl and a boy are waiting for their father''.  
    \rev{Since the hypothesis contains information (``waiting for their father'') not present in the premise image, }
    Since the description ``waiting for their father'' in the hypothesis cannot be inferred solely from the premise, the relationship is considered neutral.
\end{itemize}
% Entailment means the content of the premise logically implies the meaning of the hypothesis.
% Neutral indicates that there is no clear visual evidence in the premise to determine the truth of the hypothesis. 
% Contradiction signifies a direct conflict or inconsistency between the visual content of a premise and the meaning of a hypothesis.
% The definitions of these three classes are described in Section \ref{sec:introduction}.

% \jie{comment}
%下面这些内容能合并到上面三个类别里面吗，就类似于每个类型跟着例子说明这种。要是觉得占篇幅，不用itemize，就直接分段也可以。起码让人一目了然的get到是三个类型。
% Taking Figure \ref{fig:motivation} as an example, the premise image in the left half of Figure \ref{fig:motivation} contains a girl and a boy, which is semantically consistent with what is described in the hypothesis text, and therefore the relationship between the two is entailment.
% On the other hand, the right half of the image contains only a boy, and a girl is mentioned in the hypothesis text, which makes an obvious contradiction between the premise and the hypothesis, and therefore the relationship between the two is contradictory.
% Moreover, consider the hypothetical text "the girl and younger child are waiting for their father". 
% Because the hypothesis contains information (``waiting for their father'') not present in the premise image, the hypothesis cannot be inferred solely from the premise.
% Therefore, the relationship is considered neutral.
% \jie{comment}
%这块我觉得可以的话，可以用itemize明确的把三类列一下，可能更一目了然一些。因为你这个工作的基础就是这三类

With the development of multimodal learning, advanced VE algorithms consist of two parts.

\textbf{Feature Extraction}: extracting visual and textual features from the input premise and hypothesis, respectively;
For the extraction of premise features, the most commonly used strategy is based on object detection models.
It is based on object detection models, such as Faster R-CNN \cite{RenHG017} or YOLO \cite{RedmonDGF16}, to extract Region of Interest (RoI) features \cite{ning2018visual,cao2022alignve,YangLHMDZ22}, which means the common object in life. 
As for hypothesis features, they are usually extracted by language models such as BERT~\cite{DevlinCLT19} or LSTM~\cite{HochreiterS97}.
Then, the attention mechanism~\cite{VaswaniSPUJGKP17} is added to the features, which could focus on the semantic units of the hypothesis that corresponds to the objects on the premise.
% 2) semantic understanding: mapping the extracted features into a high-dimensional space in order to understand the semantic content of the extracted features of the image and the text;

\textbf{Relationship Prediction}: based on the extracting feature of the premise and the hypothesis, the VE model predicts whether the premise entails, contradicts, or is neutral to the hypothesis.
It typically concatenates the features of the object in the hypothesis and premise and then uses a classifier to categorize their relationship.

Therefore, in this paper, we propose that an object-centric perturbation approach could be more effective in detecting VE model issues.
% For the extraction of image features, the most commonly used strategy is based on object detection models.
% \jie{comment}
%我有个疑问是说，这种CNN的方法，是没有涉及到object的吗？如果这样的话，是不是可以直接说most commonly used strategy is based on object detection models，反正软工领域懂这个细节的也不多。这样逻辑就比较好。
%而且是否可以每说完一个part，就把这个相关的技术说了。而且在说明里面，注意突出object这个概念，这样就能让人一下子get到这个object在三个parts里面的作用。
% The first strategy utilizes Convolutional Neural Networks (CNNs) to extract global feature information from the entire image \cite{HeZRS16,ning2019visual,cao2022alignve}. 
% It is based on object detection models, such as Faster R-CNN \cite{RenHG017} or YOLO \cite{RedmonDGF16}, to extract Region of Interest (RoI) features \cite{ning2018visual,cao2022alignve,YangLHMDZ22}, which means the common object in life. 
% \jie{comment}
%这里为啥是categories，其他地方好像都没有出现object categories，都是说的object，所以要不要就说object？
% As for textual features, they are usually extracted by language models such as BERT \cite{DevlinCLT19} or LSTM \cite{HochreiterS97}.
% Then, the attention mechanism \cite{VaswaniSPUJGKP17} is added to the features, which could focus on the part of the text that corresponds to the image object.
% Inference in VE models is conducted based on the understanding of objects.


\subsection{Image Object and Semantic Unit}
\label{sec:Object_Unit}
%举例说图像中的目标和文本中的语义单元对应的一部分已经没有对应的一部分，还有文本中非语义单元的部分
%文本中非语义单元的部分往往是is这类的词，或者连词
\begin{figure}[htbp]
\centering
\includegraphics[width=8cm,height=4cm]{fig/background.png}
\caption{Examples of multiple objects in premises and hypotheses
}
\label{fig:background}
\end{figure}

We have the following two observations which can facilitate connecting text and images and designing Metamorphic Relations.

First, the scenario involves multiple objects present within both the image and the corresponding text.
As shown in subfigure a of Figure \ref{fig:background}, the text contains two words (``woman'' and ``ram'') describing the object in the image, and these two object regions also exist in the image.
Therefore, to accurately connect text with the corresponding object in the image,  it's essential to initially break down the text into multiple semantic units that describe the object in the image, like ``woman in a blue shirt is looking at a black ram'' and ``black ram''.

Second, the number of objects in the image is not consistent with the number of semantic units in the text.
As shown in subfigure b of Figure \ref{fig:background}, there are three object regions in the image, two of which correspond to ``man'' and ``rifle'' in the text, and a dog region cannot be associated with the text.
We observe that the count of objects in an image does not necessarily align with the number of semantic units in the text. 
There might be object regions or semantic units other than the associated target in the image or text. 
Therefore, after linking images and texts, it is feasible to design MRs for such unassociated objects.



Introduction-0729
\section{Introduction}
\label{sec:introduction}

% \jie{comment}
%我不是特别确定，我们这里要不要先说一两句更大一点的背景，例如大模型在各个方面整表现出卓越的能力，它的推理能力还相对比较欠缺，也是很多研究的关注重点。这其中，涉及到多模态的推理是一个更有挑战性的领域，因为他涉及到不同模态的信息理解和融合等等，VE干嘛干嘛。
%这样可能显得你这个事情更重要一些。
%写VE任务的重要性

With the rapid development of Large Language Models (LLMs), LLMs have demonstrated remarkable capabilities in various fields.
However, their inference capacities are relatively weak, which has garnered significant research attention \cite{luo2023chatgpt, Liu2023evaluate}. 
Among these, multi-modal reasoning is an especially challenging field as it involves understanding and integrating information from different modalities.
Visual Entailment (VE) is a representative task for multimodal inference.
It aims to infer about the relationship between an image and a text \cite{ning2018visual,ning2019visual}.
% Specifically,  given an image as a premise, and a natural language sentence as a hypothesis，
% the VE model understands the content of the premise and the hypothesis and determine if premise can be concluded by the hypothesis.
Specifically, given an image as the premise, and a sentence in text as the hypothesis, the Visual Entailment (VE) determines whether the hypothesis logically follows from the premise and outputs their relationship, i.e., entailment, neutral, or contradiction.
% the Visual Entailment (VE) model comprehends the contents of both the premise and the hypothesis.
% Subsequently, it 
% Specifically, given an image as a premise $P$, and a natural language sentence as a hypothesis $H$, the VE model determine if $H$ can be concluded by the $P$.
% There are three labels (entailment, neutral, contradiction) are assigned based on the relationship conveyed by the $(P, H)$.
% Entailment means the content of the $P$ logically implies the meaning of the $H$.
% Neutral indicates that there is no clear visual evidence in the $P$ to determine the truth of the $H$. 
% Contradiction signifies a direct conflict or inconsistency between the visual content of an $P$ and the meaning of a $H$.
% As the input to the VE task is multimodal data, it plays a crucial role in bridging the gap between computer vision and natural language understanding. 
As a fundamental task in the multimodal learning field, VE affects many downstream tasks such as Image Captioning~\cite{peter2018bottom,xiao2022scaling}, Visual Question Answering~\cite{stan2015vqa,Yash2019making,qing2021check}, and Image-Text Retrieval~\cite{manh2023hada}, and is applied in many real-world scenarios such as of fake news detection~\cite{Shreyash2022FACTIFY, Suryavardan2022Factify2}, medically assisted diagnosis~\cite{YanakaNCK23}, and auto-driving \cite{liang2023visual}.
Therefore, ensuring the quality of the VE model is of significant importance.

\begin{figure}[htbp]
\centering
\includegraphics[width=8cm,height=3.4cm]{fig/motivation.png}
\caption{
The origin and perturbed samples in the VE task
}
\label{fig:motivation}
\end{figure}



As the premise for the VE task, a premise contains many regions of interest that refer to different elements in the real world, such as persons, dogs, birds, etc.
Similarly, the hypothesis also describes objects and their associated properties, as well as some ancillary elements to ensure the grammaticality and fluency of the whole sentence.
% such as conjunctions and prepositions.
As reported by Xie et al, different types of elements take discrepant effects for the VE task, where the involving \textit{objects}\footnote{We follow the definition of ``objects'' for VE task in the previous study~\cite{LinMBHPRDZ14}.} serve as the foundation to infer the final relationships~\cite{ning2019visual}.
Take the sample in Figure \ref{fig:motivation} as an example.
The premise contains the three conspicuous objects, i.e., a girl, a boy, and a door, as well as their surrounding backgrounds, i.e., the wall and the floor.
While the hypothesis likewise describes two objects and their properties, i.e., ``girl stands nearby'' and ``boy sits''.
Following the general paradigm of the VE task, on the premise side, the model will detect and encode the regions of objects (the three objects framed in red) within the premise.
On the hypothesis side, the VE model will pointedly encode the key textual elements, typically referring to the objects' descriptions, using the attention mechanism.
After that, the VE will conduct relationship inference based on the semantic logic of the two-sided encoding.
Therefore, noise that occurs to the objects in either premise or the hypothesis may be more likely to result in performance fluctuation.
% Accordingly, introducing object-centric perturbations is a promising strategy for VE testing.

In recent years, many approaches are proposed for deep learning testing in the literature.
To the best of our knowledge, there are no automatic approaches for VE testing.%%%%%%%%%%%
Considering the input modalities in the VE task, the general perturbation techniques for images and texts could potentially be applied in VE testing.%第一段补一下多模态测试方法没有 --已加
However, these techniques commonly fall short when dealing with the VE task due to two aspects.
First, the vast majority of existing studies conduct semantically-equivalent perturbations, to ensure that the semantics does not change substantially while keeping the oracle unchanged.
For example, image-oriented perturbations include blurring, fogging, scaling, etc~\cite{HendrycksD19}, and text-oriented perturbations are based on synonym substitution, back translation, simulating some character-level spelling errors, or removing some uninformative words~\cite{liu2021dialtest,0002LSBLS18}.
These perturbations are relatively subtle and shallow, which can hardly affect the issue detection ability.
Especially for the VE task, ignoring the effects of objects is not likely to challenge the model's inference capacity. %intro最前面加推理能力 --已加
Second, some approaches conduct deeper perturbations, such as adding objects to the images~\cite{YuZQYWH22}, inverting the semantics of text by adding some negative words, or by antonym substitution~\cite{WangLGZZZYZZPWL21,JiangBTZD21}.
These techniques are oriented to a single modality.
% and do not consider the semantic correlation between multimodal data.
For the VE task, the arbitrary perturbations to the data on either side may break the semantic consistency with the other side, resulting in incorrect test inputs.
Generally, an object-centric perturbation considering the semantic correlation between two modalities is a crucial factor in VE testing.
% in terms of  both the correctness of test generation and the effectiveness of issue detection.



% To the best of our knowledge, there are no test approaches for VE models. 
% The input for VE models consists of data from two modalities.
% Perturbations to one modality (either image or text) can also be used in VE models. 
% \jie{comment}
%我觉得这个说法有点不太通顺，可能要加点过渡。can also be used这个逻辑有点奇怪。要不要就说，VE涉及到text和image，已有研究分别有针对image的技术和针对text的技术，然后介绍下相关技术。到最后再说目前没有同时考虑两个方面的perburbations。

\jie{comment}
%这个intro我觉得明阳老师修改的挺好的了，我还有几个小问题，
%1. 感觉上面那段说的那些技术其实也都是metamorphic testing的范畴了，就是那些perturbation其实就是通过微小变异，找到不改变output的MR。所以我觉得我们要不要就在上面那段的前面说，由于deep learning相关的应用XXX，不容易得到test oracle，所以metamorphic testing是很常用的一种方式。然后这段就说什么事就行了。
%第二，上面那段，其实是说了两大类问题，一个是变化太微小，不容易检测缺陷；二是单边的随意变化容易导致oracle变化，导致错误的结果。我觉得应该用个简洁明了的说法highlight出来，让审稿人一眼就能看到你这段表达的是什么意思，以及让他一下子就能get到做这个事情的挑战是什么，为什么已有方法不能直接用。话说上一段也挺长的，需要的话，分成两段也行。
%第三，底下这段，我看明阳先说了objects described in the hypothesis are usually a subset of objects in the premise。我感觉一下子就说这个有点思维跳跃，我觉得是不是应该一上来先说，text和image里面涉及到很多同一个元素，需要建立这种细粒度的明确的link，才能实现比较精准有效的MR。就类似于MR1，可以把两个对应的同时删掉。或者只删一端，这些不同的情况。然后再说，有些时候，因为图片是premise，图片里面的信息比较多，可能还包含其他元素，对这些元素进行变异，也会潜在影响模型的inference，等等。就类似于2.2的逻辑。当然2.2 我觉得说法上面还可以更优化一些。那两句总括性的话，还可以polish下。
%再就是，我有点觉得现在第二段，as the premise for the VE task那段，感觉是不是有点太细节了？感觉这块最后introducing object-centric perturb 后面跟着已有研究的实践，稍微有点逻辑跳跃了。我们是不是先说已有研究的问题，然后说我们需要更针对性的MR，来对这个VE进行测试。首先，我们先简单介绍下VE的基本实现，用来motivate我们的工作。然后说下这部分内容，再跟上linked object，unlinked objects那些。这样是不是逻辑更顺一点？
%我刚看了看perception matters那个工作，我觉得他intro的第二段，还挺high level的， Human cognition is believed to be a compositional process [33]: high-level reasoning and understanding requires to first perform multiple perception tasks. 就是从人的认知体系来说这个事。稍等，我再看看他怎么引到这个VQA的实现原理。
%For instance, to answer the question “is the microwave occupied?” (the second image in Fig. 1), a VQA model should first detect the microwave, extract its associated properties, identify other objects (e.g., human beings) in the context, understand the question, and try to reason about if the microwave is being used by someone. In other words, perception tasks (e.g., identifying the microwave) serve as the cornerstone for VQA models to answer high-level reasoning questions. 这个是他文章中intro 第二段的描述，我个人觉得我们在intro里面应该也是写到这种感觉。现在这块太细节了，associated properties ， ancillary elements 这些我似乎就是觉得不太需要。我觉得就是表达会识别出来objects，然后根据objects基础上进行推理这种就可以了。surrounding backgrounds啊这些就不太需要了。
%还有个细节，我觉得figure 1显得很高，都比abstract高了，所以我觉得可以把这个图上面再留白一点点，这样它看起来就会低一点了。
%我还有个问题就是，为啥sec 2 需要用两张不同的图，不能就用图1这张图吗？我只是比较好奇，不知道要说明的问题fig 1是不是有，不太清楚，再引入个新图的 是不是更好
%fig 1 里面有premise-1，premise-2，那hypothesis就不用-1，-2？或者就搞个a，b的子图，用relation做标题也行。哦，hypothesis是一样的是吧？那那个hypothesis要把 文字到图的指向画出来吗
\yuan{response}
%已经将fig 1中的图修改，sec2 的图确实用fig可以说清楚，就是图一感觉用的地方太多了，前面也对那个例子做了说明，再在background这里说那个例子会感觉有重复，background2.2这里想要表达两个意思，想分别对应两个不同的图来说。
% 此外从perception那片文章我理解的第二段要写的粒度是就从直观层面去阐述，对象是VE模型推理的基础，举例就是图像中女孩，男孩，门这三个目标，文本中有两个描述目标的语义单元，然后图像中的三个目标内容和涵盖文本语义单元，那么就是蕴含关系。然后引那片文章作为对象是推理基础的佐证就行，不从模型的角度去说具体要encode这些细节，不知道这是不是老师想表达的含义
Metamorphic testing has been widely applied to test deep learning models in the test oracle problem due to its simplicity of concept and effectiveness in issue detection~\cite{ChenKLPTTZ18}.
The core of metamorphic testing is a set of Metamorphic Relations (MRs), which are necessary properties of the tested model in relation to the inputs and their expected output.
When designing reasonable MRs for VE testing, it is essential to understand the logical relationship between object-centric perturbations and the corresponding test oracle.
Actually, objects described in the hypothesis are usually a subset of objects in the premise.
Given correspondence between premises and hypotheses, some of the objects in the premise are reflected in the hypothesis (denoted as \textit{linked objects}), while others are not (\textit{non-linked objects}).
On the one hand, perturbations to different types of objects have discriminative effects on the test oracle.
For Premise-1 in Figure \ref{fig:motivation}, the girl and the boy belong to the linked objects while the door falls non-linked ones.
If we erase a linked object in the premise and leave the hypothesis unchanged, the test oracle will change from ``entailment'' to ``contradiction''.
Otherwise, if the erasing operation occurs in the non-linked object, i.e. the door, the test oracle will remain ``entailment''.
The fact motivates us to build the object-level links between the premise and the hypothesis to distinguish different types of objects.
On the other hand, the scope of perturbations, i.e., single-side or two-side, also take significant effects on the test oracles.
Specifically, if we erase the girl in the premise and simultaneously remove the relevant description in the hypothesis (transform the original hypothesis into ``a boy sits''), the test oracle still remains ``entailment''.
Therefore, the design of the MRs should comprehensively consider the object types, perturbation scope, and their effects on the test oracles.

In this study, we propose a jointly object-centric perturbation approach (named {\tool}) for VE testing.
Generally, {\tool} identifies the objects' descriptions in the hypothesis and the objects' regions in the premise through information extraction and object detection techniques respectively.
Then, it links the objects' regions to the descriptions based on the Visual Grounding technique, while the type of each object (linked or non-linked) in the premise is determined.
After, following the framework of metamorphic testing, {\tool} designs three MRs according to the perturbation scopes (single-side or two-side), the type of the perturbed objects (linked or non-linked), and their corresponding test oracle changes.
With the MRs, {\tool} generates the new test cases for VE testing.

We evaluate the issue detection capability of {\tool} on two publicly available VE datasets, i.e, SNLI-VE~\cite{ning2018visual} and e-SNLI-VE~\cite{Virginie2020esnlive}, and take state-of-the-art VE model, OFA~\cite{WangYMLBLMZZY22} as the tested model. 
The experimental results show that the {\tool} could detect 8,537 and 10,852 issues on the two datasets respectively with 47.4\% Issue Finding Rate (IFR) on average.
And IFR is 6.6\%-40.1\% higher than the state-of-the-art baselines.
% \rev{In addition, when testing the SOTA VE models, the tests generated by the MRs in the {\tool} achieved an IFR of 76.2\%.}
Moreover, through retraining with the generated test cases, OFA could improve model robustness (0\%-0.4\% IFR) without sacrificing the accuracy on the original test set.

The key contributions of this paper are as follows:
\begin{itemize}
    \item

    Inspired by the technical principle of the VE task,  we propose a jointly object-centric perturbation approach for Visual Entailment testing.
    Particularly, different from the previous approaches, {\tool} could generate test cases based on semantic correlation between two modalities, and can motivate other research related to multimodal learning models. 

    \item 
    We evaluate {\tool} on a state-of-the-art VE model (i.e., OFA) and two widely-used datasets, the results show that {\tool} can obviously improve the issue detection ability and significantly outperforms the state-of-the-art baselines.
    
    \item
    By retraining the original OFA with the generated test cases, the model robustness could be significantly improved without sacrificing the accuracy on the original test set.
   
    \item
    We provide the public reproduction package\footnote{https://github.com/lsplx/VEtesting} including the tool implementation and datasets.
\end{itemize}

==> tab/entity_extraction_discussion.tex <==
\begin{table}[t]
\small
\caption{VG-Oriented entity extraction performance under different sizes of training samples}
\label{tab:entity_extraction}
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule
K\%  & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} &\textbf{100\%}  \\ \midrule
Precision & 82.5\%  & 85.9\%  & 87.9\%  & 88.4\%    \\
Recall  & 60.6\%  & 79.5\%  & 77.0\%  & 84.3\%      \\
F1  & 69.1\%  & 82.6\%  & 82.1\%  & 86.3\%    \\                      

\bottomrule
\end{tabular}
}
\end{table}

==> todo_list.tex <==
1. intro中的同义词变换的问题改为变换程度小
2. melt 这次词还用不用
3. image,text都改为premise和hypothesis
4.linked/non-linked 统一
5.EFR改为IFR
6.relation 改为relationship
7. erase  统一 
8.tests or test cases 统一
9.reason ability 和 infer capability
10.test approach 还是testing approach
11. test suite 还要吗
12. association  和 correaltion 统一
13. discover issue 和 detect issue 统一
14. 适用在安全领域这个描述不合适
15. object 和 object region 分别在概念和实际操作中用
16. VE task和 VE model统一
17. un-link 和non-link统一
18 joint 和jonitly统一
19.两个模型放到仓库里


issta:
1.全文改system表述
2.tests/test cases
